Program Derivation by Correctness Enhacements

Relative correctness is the property of a program to be more-correct than another program with respect to a given specification. Among the many properties of relative correctness, that which we found most intriguing is the property that program P' refines program P if and only if P' is more-correct than P with respect to any specification. This inspires us to reconsider program derivation by successive refinements: each step of this process mandates that we transform a program P into a program P' that refines P, i.e. P' is more-correct than P with respect to any specification. This raises the question: why should we want to make P' more-correct than P with respect to any specification, when we only have to satisfy specification R? In this paper, we discuss a process of program derivation that replaces traditional sequence of refinement-based correctness-preserving transformations starting from specification R by a sequence of relative correctness-based correctness-enhancing transformations starting from abort.

==> eptcsdata.tex <==
\providecommand{\firstpage}{57}
\providecommand{\publicationstatus}{Eerke Boiten, John Derrick \& Steve Reeves (Eds.):\\
Refinement Workshop 2015 (Refine '15)\\
EPTCS 209, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.209.5}{10.4204/EPTCS.209.5}}

